Online Graph Learning in Dynamic Environments

Inferring the underlying graph topology that characterizes structured data is pivotal to many graph-based models when pre-defined graphs are not available. This paper focuses on learning graphs in the case of sequential data in dynamic environments. For sequential data, we develop an online version of classic batch graph learning method. To better track graphs in dynamic environments, we assume graphs evolve in certain patterns such that dynamic priors might be embedded in the online graph learning framework. When the information of these hidden patterns is not available, we use history data to predict the evolution of graphs. Furthermore, dynamic regret analysis of the proposed method is performed and illustrates that our online graph learning algorithms can reach sublinear dynamic regret. Experimental results support the fact that our method is superior to the state-of-art methods.

==> Preliminaries/preliminaries.tex <==
We  will learn undirected  graphs $\mathcal{G}$ with non-negative  weights.  Given $N$ observed signals $\mathbf{x}_1,\ldots,\mathbf{x}_N \in \mathbb{R}^d$  generated from $\mathcal{G}$, graph learning is aimed to infer the adjacency matrix $\mathbf{A}\in \mathbb{R}^{d\times d}$ of $\mathcal{G}$. Under smoothness priors, it is equivalent to solving the following problem \cite{kalofolias2016learn}
\begin{shrinkeq}{-0.8ex}
\begin{align}
    \underset{\mathbf{A}\in \mathcal{A}}{\mathrm{min}}\; \lVert \mathbf{A} \circ \mathbf{R} \rVert_1   -\alpha \mathbf{1}^{\top}\mathrm{log}(\mathbf{A}\mathbf{1}) + \frac{\beta}{2}\lVert \mathbf{A}\rVert_{\mathrm{F}}^2,
    \label{GL-1}    
\end{align}
\end{shrinkeq}
where $\circ$ is Hadamard product and $\mathbf{1} = [1,\ldots,1]^{\top}\in \mathbb{R}^{d}$ is a vector with all entries equalling to 1. Furthermore, $\mathcal{A}$ is the adjacency matrix set defined as 
\begin{shrinkeq}{-0.5ex}
\begin{align}
        \mathcal{A} = \left\{ \mathbf{A} : \mathbf{A}\in \mathbb{R}^{d\times d}_+,  \mathbf{A} = \mathbf{A}^{\top},\mathrm{diag}(\mathbf{A}) = \mathbf{0}\right\},
    \label{GL-2}
\end{align}
\end{shrinkeq}
where $\mathbb{R}_+$ is the set of nonnegative real numbers and $\mathbf{0} \in \mathbb{R}^d$ is a vector with all entries equalling to 0. For data matrix $\mathbf{X} \in \mathbb{R}^{d\times N} = [\mathbf{x}_1,\ldots,\mathbf{x}_N] = [\tilde{\mathbf{x}}_1,\ldots,\tilde{\mathbf{x}}_d]^{\top}$, the  pairwise distance matrix $\mathbf{R}\in \mathbb{R}^{d\times d}$ in \eqref{GL-1} is defined as
\begin{shrinkeq}{-0.5ex}
\begin{align}
        \mathbf{R}_{[ij]} = \lVert \tilde{\mathbf{x}}_i - \tilde{\mathbf{x}}_j\rVert_2^2,
    \label{GL-3}   
\end{align}
\end{shrinkeq}
where $\mathbf{R}_{[ij]}$ is the $(i,j)$ entry of $\mathbf{R}$. The first term of \eqref{GL-1} is the smoothness of the observed signals over $\mathcal{G}$. Besides, the  second term controls  degrees  of  each node  while  the third  term  controls  sparsity  of  edges \cite{kalofolias2016learn}, where both $\alpha$ and $\beta$ are predefined parameters. Note that $\mathbf{A}$ is a symmetric matrix with diagonal entries equaling to 0, and hence the number of free variables of $\mathbf{A}$ is  $p\triangleq\frac{d(d-1)}{2}$. We define a vector $\mathbf{w}\in \mathbb{R}^p$ whose entries are the upper right variables of $\mathbf{A}$. Therefore, problem \eqref{GL-1} can be rewritten as
\begin{shrinkeq}{-0.5ex}
\begin{align}
       \underset{\mathbf{w}\geq 0}{\mathrm{min}} \,\, f(\mathbf{w}) =  \underset{\mathbf{w}\geq 0}{\mathrm{min}}\,\, 2\mathbf{r}^{\top}\mathbf{w} -\alpha\mathbf{1}^{\top}\mathrm{log}(\mathbf{S}\mathbf{w}) + \beta\lVert \mathbf{w} \rVert_2^2,
    \label{reformulation-of-GL-W}
\end{align}
\end{shrinkeq}
where the linear operator $\mathbf{S}$  satisfies $\mathbf{S}\mathbf{w} = \mathbf{A}\mathbf{1}$  and $\mathbf{r}$ is the vector form of the upper right variables of $\mathbf{R}$.

Under these notations, the time-varying graph learning will produce  a series of graphs $\mathbf{w}_1,\ldots,\mathbf{w}_T$ using signals $\mathbf{X}_1,\mathbf{X}_2,..\mathbf{X}_T$ collected during $T$ time periods, where $\mathbf{X}_t \in \mathbb{R}^{d\times N}$ is the data matrix of time slot $t$.  Specifically,  temporal homogeneity  assumption  based models can be formulated as 
\begin{shrinkeq}{-0.5ex}
\begin{align}
    &\underset{\mathbf{w}_t\geq 0}{\mathrm{min}}\,\, \sum_{t=1}^T f_t(\mathbf{w}_t) + \eta \sum_{t=2}^T \left\lVert\mathbf{w}_{t} - \mathbf{w}_{t-1}\right\rVert_1\notag\\[-0.2ex]
    =\,\,&\underset{\mathbf{w}_t\geq 0}{\mathrm{min}}\,\,
     2\mathbf{r}_t^{\top}\mathbf{w}_t -\alpha\mathbf{1}^{\top}\mathrm{log}(\mathbf{S}\mathbf{w}_t) + \beta\lVert \mathbf{w}_t \rVert_2^2 \notag\\[-1.5ex]
     &\quad\quad +\eta \sum_{t=2}^T \left\lVert \mathbf{w}_{t} - \mathbf{w}_{t-1}\right\rVert_1,
    \label{classic time varying graph learning}
\end{align}
\end{shrinkeq}
where $\eta$ is a global parameter controls the weight of temporal priors and $\mathbf{r}_t$ is calculated using $\mathbf{X}_t$. The last term of \eqref{classic time varying graph learning} indicates a chain structured temporal relations.






 
